Rigid and Non-rigid Shape Evolutions for Shape Alignment and Recovery in Images

The same type of objects in different images may vary in their shapes because of rigid and non-rigid shape deformations, occluding foreground as well as cluttered background. The problem concerned in this work is the shape extraction in such challenging situations. We approach the shape extraction through shape alignment and recovery. This paper presents a novel and general method for shape alignment and recovery by using one example shapes based on deterministic energy minimization. Our idea is to use general model of shape deformation in minimizing active contour energies. Given \emph{a priori} form of the shape deformation, we show how the curve evolution equation corresponding to the shape deformation can be derived. The curve evolution is called the prior variation shape evolution (PVSE). We also derive the energy-minimizing PVSE for minimizing active contour energies. For shape recovery, we propose to use the PVSE that deforms the shape while preserving its shape characteristics. For choosing such shape-preserving PVSE, a theory of shape preservability of the PVSE is established. Experimental results validate the theory and the formulations, and they demonstrate the effectiveness of our method.

==> bak.tex <==
\section{What energy functional can be minimized by curve evolution?}\label{SEC:BAK}
%\subsection{Deterministic models of shape deformations: warping and curve evolution}
%This paper addresses the deformation of the boundary contour of the 2D shape silhouette. The mathematical definition of the boundary contour is $C(p)=\mathbf{x}(p)=[x_1(p),x_2(p)]^T$, $\mathbf{x}(p)\in C\subset R^2$, where $p$ is the parametrization. Sometimes, the silhouette may contain holes, and the corresponding boundary is a set of multiple closed curves, but the above formulation of $C(p)$ can model the multiple closed curves by incorporation some discontinuities in $C(p)$ w.r.t. $p$. When integrating/differentiating $C(p)$ w.r.t. $p$, we can decompose the integral/differential into multiple parts to avoid the discontinuities. We shall omit this trivial treatment in the following for conciseness.
%
%The warping transformation of the boundary contour $C(p)=\mathbf{x}(p)$, which we refer to as the shape warping, can be formulated as follows.
%\begin{equation}\label{EQ:Warp1}
%\mathbf{\tilde{x}}(p) = \mathbf{f}(\mathbf{x}(p),\theta),
%\end{equation}
%where $\mathbf{f}$ is the warping mapping, $\mathbf{\tilde{x}(p)}$ is the transformed boundary point, $\theta$ can be a vector of parameters. This defines the boundary warping.
%
%When the warping mapping is differentiable, thus we can redefine the warping in Eq. (\ref{EQ:Warp1}) by the Taylor expansion as follows.
%\begin{equation}\label{EQ:Warp2}
%\mathbf{\tilde{x}}(p) = \mathbf{x}(p)+ \left.\left[{\mathbf{D}\mathbf{f}(\mathbf{x}(p),\theta)\over\mathbf{D}\theta}\right|_{\theta=0}\right]\theta + O(\theta),
%\end{equation}
%where $\mathbf{D}$ is the multivariate differential operator. Let $\mathbf{x}(p,\theta) = \mathbf{\tilde{x}}(p)$ and $\mathbf{x}_0(p) = \mathbf{x}(p)$, we can rewrite the above as follows.
%\begin{equation}\label{EQ:Warp3}
%\mathbf{x}(p,\theta) = \mathbf{x}(p,0)+ \left.\left[{\mathbf{D}\mathbf{f}(\mathbf{x}(p,0),\theta)\over\mathbf{D}\theta}\right|_{\theta=0}\right]\theta + O(\theta),
%\end{equation}
%which depicts the infinitesimal dynamics of the shape warping. A special case of this idea is the infinitesimal transform [??] in the following.
%\begin{equation}\label{EQ:infsmal_trans}
%\mathbf{x}(p,\epsilon) = \mathbf{x}(p,0)+ \epsilon\mathbf{A}\mathbf{x}(p,0), \hbox{for}~ \epsilon\rightarrow 0,
%\end{equation}
%where $\mathbf{A}$ is an constant matrix, $\epsilon$ is an infinitesimal scalar. We can observe the consistency between the infinitesimal transform and the Taylor expansion of a general warping transformation. In fact, the Taylor expansion of linear warping transformations, such as the rotation, scaling etc., can be written in the form of the infinitesimal transform as follows.
%\begin{equation}\label{EQ:infsmal_Rot}
%\begin{split}
%\mathbf{x}(p,\omega) &= \left[\begin{array}{cc}
%                          \cos(\omega)  & \sin(\omega) \\
%                          -\sin(\omega) & \cos(\omega)
%                        \end{array}\right]
%\mathbf{x}(p,0) \\
%                     &= \mathbf{x}(p,0)+ \omega\left[\begin{array}{cc}
%                          0  & 1 \\
%                          -1 & 0
%                        \end{array}\right]\mathbf{x}(p,0)+O(\omega),
%\end{split}
%\end{equation}
%The infinitesimal transformation is the linearization of the nonlinear deformations, which is useful for analyzing nonlinear dynamic systems \cite{Khalil02Nonlinear}.
%
%Curve evolution equation, as follows, can also be viewed as a dynamic model of shape deformation.
%\begin{equation}
%\begin{split}
%{\partial C(p,t)\over\partial t} = \alpha(p,t)\mathbf{N}(p,t)+\beta(p,t)\mathbf{T}(p,t)&,\\
%C(p,0)=C_0&,\\
%\end{split}
%\end{equation}
%where $t$ is an artificial time of the curve evolution, $\mathbf{N}(p,t)$ is the normal vector of the curve, $\mathbf{T}(p,t)$ is the tangential vector of the curve, $\alpha(p,t),\beta(p,t)$ are projections of the evolving velocity on the normal and tangential directions, $C_0$ is the initial curve. Moreover, since the tangential velocity cannot affect the geometry of the curve evolution [], the above can be simplified to be the following.
%\begin{equation}\label{EQ:CE}
%{\partial C(p,t)\over\partial t} = \alpha(p,t)\mathbf{N}(p,t),~~C(p,0)=C_0
%\end{equation}
%
%The direct solution to the above curve evolution equation requires the artificial reparametrization. It is numerically more advantageous to solve the curve evolution equation by level set method \cite{OsherSethian88Fronts}. The motivation of the level set method is the implicit representation of contour by functions, e.g. $C(p,t)=\{x,y|\phi(x,y,t)=0\}$, $\phi(x,y,t)$ is normally a signed distance function. By differentiating $\phi(x,y,t)=0$ w.r.t. $t$, we obtain the following famous level set equation.
%\begin{equation}\label{EQ:LS1}
%\begin{split}
%{\partial \phi(x,y,t)\over\partial t} = \nabla\phi(x,y,t)\cdot\left[{dx\over d t},{dy\over d t}\right]^T&,\\
%\phi(x,y,0)=\phi_0(x,y)&,
%\end{split}
%\end{equation}
%for $\nabla=\left[{\partial\over\partial x},{\partial\over\partial y}\right]^T$, $[x,y]^T\in C(p,t)$, and the $\phi$ at some time is defined as follows.
%\begin{equation}\label{EQ:SDF}
%\begin{split}
%\phi(\mathbf{x}) = \left\{\begin{array}{rl}
%                d(\mathbf{x},C) &  \mathbf{x}\in \Omega\\
%                -d(\mathbf{x},C) &  \mathbf{x}\notin \Omega
%              \end{array}\right.
%\end{split}
%\end{equation}
%where $\Omega$ is the region defined by the closed contours $C$, such that $C$ is the boundary of $\Omega$, $d$ is the Euclidean distance from a point to the curve $C$. $\phi_0$ is the signed distance function defined in terms of $C_0$.
%%Knowing that the following holds,
%%\begin{equation}
%%\left[{dx\over dt},{dy\over dt}\right]^T = {dC(p,t)\over dt}={\partial C\over \partial p}{dp\over dt}+{\partial C\over \partial t},
%%\end{equation}
%%but the level set equation Eq. (\ref{EQ:LS1}) only depends on ${\partial C\over \partial t}$, since ${\partial C\over \partial p}\cdot\mathbf{N}=0$ and $\nabla\phi(x,y,t)=-\mathbf{N}$.
%
%After some derivations, the resultant level set equation for the curve evolution Eq. (\ref{EQ:CE}) can be written as follows.
%\begin{equation}\label{EQ:LS2}
%\begin{split}
%{\partial \phi(x,y,t)\over\partial t} = -\alpha(x,y,t)\Big\|\nabla\phi(x,y,t)\Big\|&,\\
%\phi(x,y,0)=\phi_0(x,y)&,
%\end{split}
%\end{equation}
%where $\alpha(x,y,t)=\alpha(p(x),p(y),t)$, knowing that $C(p)$ is invertible.
%
%The general formulation of curve evolution equation allows the shape to deform arbitrarily, whereas the shape warping by using the warping mapping chosen \emph{a priori} can restrict the deformation. Hence, we consider that the shape warping is a better model of shape deformation than the curve evolution equation.

%\subsection{Active contour model, the calculus of variation and the curve evolution}
%Although shape warping can be better for modeling shape deformation, curve evolution equations can be used to solve active contours, whereas the active contours based on shape warping is not obvious.

The active contour model in its contour-integral form, i.e. the boundary based active contour, can be written as follows.
\begin{equation}\label{EQ:Gen_AC1}
C^*(p) = \argmin\limits_{C(p)} \mathcal{J}(C) = \int_C g(C,C_p,C_{pp},...,) dp
\end{equation}
where $p$ denotes the parametrization of the contour, $g$ is a function mapping, $C_p={\partial \over\partial p}C$, $C_{pp}={\partial^2 \over\partial p^2}C$ etc., are the partial derivatives of the contour $C_p$. Snakes model was formulated in this form. A drawback of this model is that the energy of $\mathcal{J}$ can vary by changing the parametrization.

An alternative to the Snakes is the geodesic active contour (GAC) \cite{caselles97GAC} \cite{Yezzi97GAC_J} in the following form.
\begin{equation}\label{EQ:Gen_AC2}
C^* = \argmin\limits_{C} \mathcal{J}^C(C) = \int_C g(C)\|C_p\| dp =  \int_C g(C) ds
\end{equation}
where $ds = \|C_p\|dp$ is the arc-length parametrization. The GAC energy does not vary for different parameterizations by $p$. This can also be verified by the following striking equivalence.
\begin{equation}\label{EQ:Gen_AC3}
\mathcal{J}^C(C) = \int_C g(C) ds = \int_\mathcal{D} g(x,y)\delta(\phi)\|\nabla\phi\|dxdy
\end{equation}
which transforms a contour integral into a region integral due to the coarea formula \cite{Evans92Measure}, where $\mathcal{D}$ is the entire integral domain, $\delta(\cdot)$ is a Dirac delta function, $\phi$ is a signed distance function defined as follows.
\begin{equation}\label{EQ:SDF}
\begin{split}
\phi_{_\Omega}(x,y) = \left\{\begin{array}{rl}
                d([x,y]^T,C) &  [x,y]^T\in \Omega\\
                -d([x,y]^T,C) &  [x,y]^T\notin \Omega
              \end{array}\right.
\end{split}
\end{equation}
where $\Omega$ is the region enclosed by $C$, $d([x,y]^T,C)$ is the Euclidean distance from $[x,y]^T$ to the curve $C$. (\ref{EQ:Gen_AC3}) tells that the GAC in a contour integral form is equivalent to a region integral, which only depends on the \emph{shape} of the contour.

Contour integral can only measure the optimality of the contour according to the local image features. The active contour models can also be directly formulated as region integrals that measure the optimality of contour according to the regional properties of the inner and outer regions of the contour, such as \cite{Zhusongchun96RegComp} \cite{ChanVese01ActiveCon} \cite{Brox2009InterpMumfordShah}. The general active contour in the region integral form is as follows.
\begin{equation}\label{EQ:OptDomain}
\Omega^* = \argmin\limits_{\Omega} \mathcal{J}^\Omega(\Omega),
\end{equation}
and,
\begin{equation}\label{EQ:DomainInt}
\begin{split}
\mathcal{J}^\Omega(\Omega) &= \gamma_1\int_{_\Omega} g(x,y) dxdy+\gamma_2\int_{\mathcal{D}\setminus{\Omega}} \bar{g}(x,y) dxdy,
 \end{split}
\end{equation}
where $\Omega\in \mathcal{D}$ is the region to optimize, $\mathcal{D}$ is the entire integral domain,  $g(x,y)$ and $\bar{g}(x,y)$ are function mappings defined over the entire domain, $\phi_{_\Omega}(x,y)$ is a signed distance function defined in Eq. (\ref{EQ:SDF}) in which $\Omega$ is the region defined by the closed contours $C$, such that $C$ is the boundary of $\Omega$. Besides, the $\gamma_1,\gamma_2$ are penalty coefficients.

To facilitate the derivations, we may follow the conventions in Chan-Vese model to reformulate Equations (\ref{EQ:OptDomain}) and (\ref{EQ:DomainInt}) as follows.
\begin{equation}\label{EQ:OptDomain_}
\phi_{_\Omega}^* = \argmin\limits_{\phi_{_\Omega}} \mathcal{\hat{J}}^\Omega(\phi_{_\Omega}),
\end{equation}
and,
\begin{equation}\label{EQ:DomainInt_}
\begin{split}
\mathcal{\hat{J}}^\Omega(\phi_{_\Omega}) &= \gamma_1\int_{\mathcal{D}} g(x,y)H(\phi_{_\Omega}) dxdy\\
 &\hspace{10pt}+ \gamma_2\int_{\mathcal{D}} \bar{g}(x,y)(1-H(\phi_{_\Omega})) dxdy,
\end{split}
\end{equation}
where $H(\cdot)$ is a 1-D Heaviside function.

Since the GAC model can also be written in a region integral form, we can combine (\ref{EQ:Gen_AC3}) and (\ref{EQ:OptDomain_}) to obtain the following joint boundary-region based active contour.
\begin{equation}\label{EQ:OptDomain_final}
\phi_{_\Omega}^* = \argmin\limits_{\phi_{_\Omega}} \mathcal{G}(\phi_{_\Omega}),
\end{equation}
and,
\begin{equation}\label{EQ:DomainInt_final}
\begin{split}
\mathcal{G}(\phi_{_\Omega}) &= \gamma_1\int_{\mathcal{D}} \hat{g}(x,y) \delta(\phi_{_\Omega})dxdy\\
 &\hspace{0.3in}+\gamma_2\int_{\mathcal{D}} g(x,y)H(\phi_{_\Omega}) dxdy\\
  &\hspace{0.3in}+ \gamma_3\int_{\mathcal{D}} \bar{g}(x,y)(1-H(\phi_{_\Omega})) dxdy,
 \end{split}
\end{equation}
where $\gamma_1,\gamma_2,\gamma_3$ are penalty coefficients

\begin{figure*}[!t]
%\vspace*{1pt}
%\hrulefill
\normalsize
\begin{equation}\label{EQ:D_DomainInt_final}
\begin{split}
%{d\mathcal{G}(\phi_{_\Omega}(x,y,t))\over dt} &= \gamma_1\int_{\mathcal{D}}\left[\left\langle\nabla g,{\nabla\phi_{_\Omega}\over\|\nabla\phi_{_\Omega}\|}\right\rangle + g \nabla\cdot\left({\nabla\phi_{_\Omega}\over\|\nabla\phi_{_\Omega}\|}\right)\right] \delta(\phi_{_\Omega}){d\phi\over d t}dxdy\\
% &+\gamma_2\int_{\mathcal{D}} g(x,y)\delta(\phi_{_\Omega}) {d\phi\over d t}dxdy - \gamma_3\int_{\mathcal{D}} \bar{g}(x,y)\delta(\phi_{_\Omega}){d\phi\over d t} dxdy,
{d\mathcal{G}(\phi_{_\Omega}(x,y,t))\over dt} &= \gamma_1\int_{C}\Big[\left\langle\nabla \hat{g},\mathbf{N}\right\rangle - \hat{g} \nabla\cdot\mathbf{N}\Big] \left\langle\mathbf{N},{\partial C(s,t)\over\partial t}\right\rangle ds\\
 &\hspace{0.3in}+\gamma_2\int_{C} g(x,y)\left\langle\mathbf{N},{\partial C(s,t)\over\partial t}\right\rangle ds - \gamma_3\int_{C} \bar{g}(x,y)\left\langle\mathbf{N},{\partial C(s,t)\over\partial t}\right\rangle ds
 \end{split}
\end{equation}
\hrulefill
\end{figure*}

The problem (\ref{EQ:OptDomain_final}) is known as the optimization of domain integral in the literature of optimal shape design \cite{BookPrincOptDes}. The global optimization method is generally prohibitive due to the infinite many dimensions in theory and the indefinitely many dimensions by discretization. The conventional technique to solve this problem is the calculus of shape gradient by using the cumbersome transformation of variables \cite{BookPrincOptDes} \cite{Aubert03ShapeGrad}. A more advanced derivation is due to the level set calculus with the help of the coarea formula \cite{Evans92Measure} \cite{Burger05Asurvey} \cite{Fedkiw03OsherContrib} based on functional differentiations (the calculus of variations), i.e. the $G\hat{a}teaux$ and $Fr\acute{e}chet$ derivatives. Interested readers may refer to \cite{Book74CoV2PhyEng} for fundamentals and motivating applications of the calculus of variations, and to \cite{Book09FunctionalNumerical} for an outline of the theory of functional derivatives.

The level set calculus presented in \cite{Burger05Asurvey} provides us Eq. (\ref{EQ:D_DomainInt_final}), in which $\mathbf{N}={\nabla\phi_{_\Omega}/\|\nabla\phi_{_\Omega}\|}$ is the normal of the boundary curve $C$, $\phi_{_\Omega}$ is defined in Equation (\ref{EQ:SDF}), $s$ is the arc-length parametrization. Eq. (\ref{EQ:D_DomainInt_final}) is not really a novel result. Eq. (\ref{EQ:D_DomainInt_final}) tells that both the contour or region integral can be altered by a variation in the boundary $C$. Accordingly, we may rewrite Eq. (\ref{EQ:D_DomainInt_final}) in the following concise form.
\begin{equation}\label{EQ:D_RInt2CE}
{d\mathcal{G}(\phi_{_\Omega}(x,y,t))\over dt} = \int_{C} \left\langle\nabla \mathcal{G}(C),{\partial C(s,t)\over\partial t}\right\rangle ds,
\end{equation}
where $\nabla\mathcal{G}(C)= g_{_D}(C)\mathbf{N}$, $g_{_D}(C)$ is a scalar function defined on $C$. The gradient descent curve evolution equation is as follows.
\begin{equation}\label{EQ:CE_RInt}
{\partial C(s,t)\over\partial t}=-g_{_D}(C)\mathbf{N}, ~~C(s,0)=C_0(s).
\end{equation}
The above leads to energy minimization as follows.
\begin{equation}\label{EQ:Dt_Gen_AC}
{d\mathcal{G}\over dt} =  -\int_p\|g_{_D}(C)\|^2dp\leq0.
\end{equation}

All the above implies that both the boundary and region based active contour energy functionals in (\ref{EQ:Gen_AC3}) and (\ref{EQ:DomainInt}) can be minimized by curve evolution, given an initial contour curve. The numerical implementation of the curve evolution is often due to the level set method \cite{OsherSethian88Fronts} to avoid the contour reparametrization during the curve evolution.

Our major question regarding the simultaneous object segmentation and shape recovery is: \emph{does there exist a deformable shape model in the form of curve evolution equation for minimizing the the active contour energy}.

%
%
%
%
%
%
%
%According to the definition of $G\hat{a}teaux$ derivative, we can perform the functional analogy of directional derivative for Eq. (\ref{EQ:Gen_AC}) to yield the following.
%\begin{equation}\label{EQ:Dir_Gen_AC}
%\left.{d\mathcal{J}(C+\epsilon\eta)\over d\epsilon}\right|_{\epsilon=0} = \Big\langle\nabla \mathcal{J},\eta\Big\rangle^*_p = \int_C \langle\nabla \mathcal{J},\eta\rangle dp,
%\end{equation}
%where $\langle,\rangle^*_p$ is the $L_2$ inner product of 2D vectorial functions defined along the parametrization $p$ of the curve $C$, the later $\langle,\rangle$ is a conventional vector inner product , $\eta(p)$ is the so-called variation of function $C(p)$, $\nabla \mathcal{J}(C)$ is the functional gradient of the functional $\mathcal{J}(C)$. The stationary condition for the optimality is therefore the $\nabla \mathcal{J}=0$, which is the famous Euler-Lagrange equation, and the directional differentiation of functional is the calculus of variation. Interesting fundamental discussions of the calculus of variations can be found in \cite{Book74CoV2PhyEng}.
%
%The gradient descent equation is also the analogy to the finite dimensional case as follows.
%\begin{equation}
%{\partial C(p,t)\over\partial t} = -\nabla \mathcal{J},~~C(p,0)=C_0(p).
%\end{equation}
%
%The geometry of the above gradient descent equation is equivalent to the following \cite{Epstein87CS}.
%\begin{equation}\label{EQ:CE_Gen_AC}
%{\partial C(p,t)\over\partial t} = -\langle\nabla \mathcal{J},\mathbf{N}\rangle\mathbf{N},~~
%C(p,0)=C_0(p).
%\end{equation}
%
%Why does this curve evolution decrease the functional energy $J$? This question can be answered by differentiating $\mathcal{J}(C)$ w.r.t. the $t$ as follows.
%\begin{equation}\label{EQ:Dt_Gen_AC}
%\begin{split}
%{d\mathcal{J}(C(p,t))\over dt} &= \left\langle\nabla \mathcal{J},{\partial C(p,t)\over\partial t}\right\rangle^*_p\\
% &= -\int_p\|\langle\nabla \mathcal{J},\mathbf{N}\rangle\|^2dp\leq0,
%\end{split}
%\end{equation}
%where we have assumed ${dp\over dt}=0$ to prohibit change of parametrization (different from the reparametrization in numerical implementation). Sometimes, $\mathcal{J}(C)$ can be formulated such that the change of parametrization does not affect the energy, i.e. $\Big\langle\nabla \mathcal{J},{\partial C(p,t)\over\partial p}\Big\rangle^*_p=0$, such as the Geodesic Active Contour \cite{caselles97GAC} \cite{Kichenassamy96GAC}. The numerical implementation of the curve evolution is often by the level set method \cite{OsherSethian88Fronts}, which does not require reparametrization of the curve during the curve evolution. 

==> unif.tex <==
\subsection{Minimizing region based active contours by curve evolution}
In Eq. (\ref{EQ:Gen_AC}), the boundary based active contour model is a contour integral which can vary according to the curve evolution. However, contour integral can only measure the optimality of the contour according to the local image features. The active contour models can be formulated as region integrals that measure the optimality of contour according to the inner and outer regions of the contour. Interestingly, the active contour models in terms of region integrals are also often solved by curve evolution \cite{Zhusongchun96RegComp} \cite{ChanVese01ActiveCon} \cite{Brox2009InterpMumfordShah}. In this section, we present the general formulations that accomplish the unification of the boundary based and region based active contours through curve evolution, which also provides the theoretical foundation of using curve evolution, instead of conventional warping mapping, for shape registration.

The general active contour in the region integral form as follows.
\begin{equation}\label{EQ:OptDomain}
\Omega^* = \argmin\limits_{\Omega} \mathcal{G}(\Omega),
\end{equation}
and,
\begin{equation}\label{EQ:DomainInt}
\begin{split}
\mathcal{G}(\Omega) &= \gamma_1\int_{\mathcal{D}} \hat{g}(x,y) \delta(\phi_{_\Omega}(x,y))dxdy\\
 &+\gamma_2\int_{_\Omega} g(x,y) dxdy + \gamma_3\int_{\mathcal{D}\setminus{\Omega}} \bar{g}(x,y) dxdy,
 \end{split}
\end{equation}
where $\Omega\in \mathcal{D}$ is the region to optimize, $\mathcal{D}$ is the entire integral domain,  $\hat{g}(x,y)$, $g(x,y)$ and $\bar{g}(x,y)$ are function mappings defined over the entire domain, $\phi_{_\Omega}(x,y)$ is a signed distance function defined in Eq. (\ref{EQ:SDF}) in which $\Omega$ is the region defined by the closed contours $C$, such that $C$ is the boundary of $\Omega$. Besides, $\delta(\cdot)$ is a Dirac delta function, $\gamma_1,\gamma_2,\gamma_3$ are penalty coefficients.

The problem (\ref{EQ:OptDomain}) is known as the optimization of domain integral in the literature of optimal shape design \cite{BookPrincOptDes}. The conventional technique to solve this problem is the calculus of shape gradient by using the cumbersome transformation of variables \cite{BookPrincOptDes} \cite{Aubert03ShapeGrad}. A more advanced derivation is due to the level set calculus with the help of the coarea formula \cite{Evans92Measure} \cite{Burger05Asurvey} \cite{Fedkiw03OsherContrib}. To allow the level set calculus, we reformulate Eqs. (\ref{EQ:OptDomain}) and (\ref{EQ:DomainInt}) as follows.
\begin{equation}\label{EQ:OptDomain}
\phi_{_\Omega}^* = \argmin\limits_{\phi_{_\Omega}} \mathcal{G}(\phi_{_\Omega}),
\end{equation}
and,
\begin{equation}\label{EQ:DomainInt}
\begin{split}
\mathcal{G}(\phi_{_\Omega}) &= \gamma_1\int_{\mathcal{D}} \hat{g}(x,y) \delta(\phi_{_\Omega})dxdy\\
 &\hspace{0.3in}+\gamma_2\int_{\mathcal{D}} g(x,y)H(\phi_{_\Omega}) dxdy\\
  &\hspace{0.3in}+ \gamma_3\int_{\mathcal{D}} \bar{g}(x,y)(1-H(\phi_{_\Omega})) dxdy,
 \end{split}
\end{equation}
where $H(\cdot)$ is a 1-D Heaviside function.

The level set calculus provides us Eq. (\ref{EQ:D_DomainInt}), in which $\mathbf{N}=-{\nabla\phi_{_\Omega}/\|\nabla\phi_{_\Omega}\|}$ is the normal of the boundary curve $C$, $s$ is the arclenth parametrization. Eq. (\ref{EQ:D_DomainInt}) is not really a novel result which can be found in \cite{Burger05Asurvey}. Eq. (\ref{EQ:D_DomainInt}) tells that a change of the region integral is due to a variation in the boundary. Eq. (\ref{EQ:D_DomainInt}) implies that the region based active contour defined in Eq. (\ref{EQ:DomainInt}) can be optimized by curve evolution, given an initial contour curve.
\begin{figure*}[!t]
%\vspace*{1pt}
%\hrulefill
\normalsize
\begin{equation}\label{EQ:D_DomainInt}
\begin{split}
%{d\mathcal{G}(\phi_{_\Omega}(x,y,t))\over dt} &= \gamma_1\int_{\mathcal{D}}\left[\left\langle\nabla g,{\nabla\phi_{_\Omega}\over\|\nabla\phi_{_\Omega}\|}\right\rangle + g \nabla\cdot\left({\nabla\phi_{_\Omega}\over\|\nabla\phi_{_\Omega}\|}\right)\right] \delta(\phi_{_\Omega}){d\phi\over d t}dxdy\\
% &+\gamma_2\int_{\mathcal{D}} g(x,y)\delta(\phi_{_\Omega}) {d\phi\over d t}dxdy - \gamma_3\int_{\mathcal{D}} \bar{g}(x,y)\delta(\phi_{_\Omega}){d\phi\over d t} dxdy,
{d\mathcal{G}(\phi_{_\Omega}(x,y,t))\over dt} &= \gamma_1\int_{C}\Big[\left\langle\nabla \hat{g},-\mathbf{N}\right\rangle + \hat{g} \nabla\cdot\mathbf{N}\Big] \left\langle-\mathbf{N},{\partial C(s,t)\over\partial t}\right\rangle ds\\
 &\hspace{0.3in}+\gamma_2\int_{C} g(x,y)\left\langle-\mathbf{N},{\partial C(s,t)\over\partial t}\right\rangle ds - \gamma_3\int_{C} \bar{g}(x,y)\left\langle-\mathbf{N},{\partial C(s,t)\over\partial t}\right\rangle ds
 \end{split}
\end{equation}
\hrulefill
\end{figure*}

Accordingly, we may rewrite Eq. (\ref{EQ:D_DomainInt}) in the following form.
\begin{equation}\label{EQ:D_RInt2CE}
{d\mathcal{G}(\phi_{_\Omega}(x,y,t))\over dt} = \int_{C} \left\langle\nabla \mathcal{G}(C),{\partial C(s,t)\over\partial t}\right\rangle ds,
\end{equation}
where $\nabla\mathcal{G}(C)= g_{_D}(C)\mathbf{N}$, $g_{_D}(C)$ is a scalar function defined on $C$. Similar to Eq. (\ref{EQ:Dt_Gen_AC}), if we set
\begin{equation}\label{EQ:CE_RInt}
{\partial C(s,t)\over\partial t}=-g_{_D}(C)\mathbf{N}, ~~C(s,0)=C_0(s),
\end{equation}
we have ${d\mathcal{G}(\phi_{_\Omega}(x,y,t))\over dt}\leq0$.

To conclude, minimizing the active contour energy generally requires curve evolution equation. Our major question is: \emph{can the optimal contour due to curve evolution be controlled similar to the user-specified prototype shape contour?}

